Regression Discontinuity Design with Distribution-Valued Outcomes

This article introduces Regression Discontinuity Design (RDD) with Distribution-Valued Outcomes (R3D), extending the standard RDD framework to settings where the outcome is a distribution rather than a scalar. Such settings arise when treatment is assigned at a higher level of aggregation than the outcome-for example, when a subsidy is allocated based on a firm-level revenue cutoff while the outcome of interest is the distribution of employee wages within the firm. Since standard RDD methods cannot accommodate such two-level randomness, I propose a novel approach based on random distributions. The target estimand is a "local average quantile treatment effect", which averages across random quantiles. To estimate this target, I introduce two related approaches: one that extends local polynomial regression to random quantiles and another based on local Fr\'echet regression, a form of functional regression. For both estimators, I establish asymptotic normality and develop uniform, debiased confidence bands together with a data-driven bandwidth selection procedure. Simulations validate these theoretical properties and show existing methods to be biased and inconsistent in this setting. I then apply the proposed methods to study the effects of gubernatorial party control on within-state income distributions in the US, using a close-election design. The results suggest a classic equality-efficiency tradeoff under Democratic governorship, driven by reductions in income at the top of the distribution.

==> figs/standard_rd_results.tex <==

\begin{tabular}{lcc}
\hline\hline
 & \multicolumn{1}{c}{Aggregated} & \multicolumn{1}{c}{Family Level} \\
\hline
Treatment Effect & -0.631 & -0.525 \\
 & (0.419) & (0.062) \\
\\
Robust 95\% CI & [-1.537, 0.105] & [-0.681, -0.438] \\
p-value & 0.087 & 0 \\
Bandwidth & 0.083 & 0.036 \\
Effective Observations & 203 & 138692 \\
\hline\hline
\end{tabular}

==> tabs/combined_cp_table_scenario_1.tex <==
\begin{table}[!h]
\centering
\caption{Coverage and Power Metrics for Scenario 1}
\centering
\begin{tabular}[t]{l|r|r|r|r|r|r}
\hline
\multicolumn{2}{c|}{ } & \multicolumn{3}{c|}{Uniform Bands} & \multicolumn{2}{c}{Tests} \\
\cline{3-5} \cline{6-7}
Method & Sample\_Size & Joint Coverage (\%) & Avg Coverage (\%) & Avg Power (\%) & Power Nullity (\%) & Power Homogeneity (\%)\\
\hline
\cellcolor{gray!10}{R3D Frechet} & \cellcolor{gray!10}{200} & \cellcolor{gray!10}{87.0} & \cellcolor{gray!10}{91.5} & \cellcolor{gray!10}{32.6} & \cellcolor{gray!10}{41.0} & \cellcolor{gray!10}{12.2}\\
\hline
R3D Frechet & 500 & 92.8 & 94.8 & 55.6 & 61.8 & 10.4\\
\hline
\cellcolor{gray!10}{R3D Local Polynomial} & \cellcolor{gray!10}{200} & \cellcolor{gray!10}{86.0} & \cellcolor{gray!10}{92.0} & \cellcolor{gray!10}{29.2} & \cellcolor{gray!10}{40.8} & \cellcolor{gray!10}{12.0}\\
\hline
R3D Local Polynomial & 500 & 91.6 & 95.4 & 51.9 & 61.8 & 13.0\\
\hline
\end{tabular}
\end{table}

==> tabs/coverage_power_table_scenario_2.tex <==
\begin{table}[!h]
\centering
\caption{Coverage and Power for Scenario 2}
\centering
\begin{tabular}[t]{r|r|r|r|r|r|r|r|r|r}
\hline
\multicolumn{2}{c|}{ } & \multicolumn{4}{c|}{Coverage (\%)} & \multicolumn{4}{c}{Power (\%)} \\
\cline{3-6} \cline{7-10}
Method & Sample\_Size & Average & Q25 & Q50 & Q75 & Average & Q25 & Q50 & Q75\\
\hline
\cellcolor{gray!10}{Quantile RD} & \cellcolor{gray!10}{200} & \cellcolor{gray!10}{NaN} & \cellcolor{gray!10}{NaN} & \cellcolor{gray!10}{NaN} & \cellcolor{gray!10}{NaN} & \cellcolor{gray!10}{NaN} & \cellcolor{gray!10}{NaN} & \cellcolor{gray!10}{NaN} & \cellcolor{gray!10}{NaN}\\
\hline
Quantile RD & 500 & NaN & NaN & NaN & NaN & NaN & NaN & NaN & NaN\\
\hline
\cellcolor{gray!10}{R3D Frechet} & \cellcolor{gray!10}{200} & \cellcolor{gray!10}{25.4} & \cellcolor{gray!10}{24.4} & \cellcolor{gray!10}{27.0} & \cellcolor{gray!10}{30.8} & \cellcolor{gray!10}{99.5} & \cellcolor{gray!10}{99.4} & \cellcolor{gray!10}{99.6} & \cellcolor{gray!10}{99.6}\\
\hline
R3D Frechet & 500 & 15.9 & 14.4 & 19.8 & 19.8 & 99.9 & 99.8 & 99.8 & 100.0\\
\hline
\cellcolor{gray!10}{R3D Local Polynomial} & \cellcolor{gray!10}{200} & \cellcolor{gray!10}{27.4} & \cellcolor{gray!10}{27.2} & \cellcolor{gray!10}{30.2} & \cellcolor{gray!10}{30.8} & \cellcolor{gray!10}{99.5} & \cellcolor{gray!10}{99.4} & \cellcolor{gray!10}{99.6} & \cellcolor{gray!10}{99.6}\\
\hline
R3D Local Polynomial & 500 & 18.1 & 16.4 & 23.0 & 21.6 & 99.9 & 99.8 & 99.8 & 100.0\\
\hline
\end{tabular}
\end{table}

==> tabs/coverage_power_table_scenario_3.tex <==
\begin{table}[!h]
\centering
\caption{Coverage and Power for Scenario 3}
\centering
\begin{tabular}[t]{r|r|r|r|r|r|r|r|r|r}
\hline
\multicolumn{2}{c|}{ } & \multicolumn{4}{c|}{Coverage (\%)} & \multicolumn{4}{c}{Power (\%)} \\
\cline{3-6} \cline{7-10}
Method & Sample\_Size & Average & Q25 & Q50 & Q75 & Average & Q25 & Q50 & Q75\\
\hline
\cellcolor{gray!10}{Classical QTE.RD} & \cellcolor{gray!10}{100} & \cellcolor{gray!10}{NaN} & \cellcolor{gray!10}{NaN} & \cellcolor{gray!10}{NaN} & \cellcolor{gray!10}{NaN} & \cellcolor{gray!10}{NaN} & \cellcolor{gray!10}{NaN} & \cellcolor{gray!10}{NaN} & \cellcolor{gray!10}{NaN}\\
\hline
Classical QTE.RD & 200 & NaN & NaN & NaN & NaN & NaN & NaN & NaN & NaN\\
\hline
\cellcolor{gray!10}{Classical QTE.RD} & \cellcolor{gray!10}{500} & \cellcolor{gray!10}{NaN} & \cellcolor{gray!10}{NaN} & \cellcolor{gray!10}{NaN} & \cellcolor{gray!10}{NaN} & \cellcolor{gray!10}{NaN} & \cellcolor{gray!10}{NaN} & \cellcolor{gray!10}{NaN} & \cellcolor{gray!10}{NaN}\\
\hline
R3D Frechet & 100 & 6052.6 & 7500 & 6500 & 5000 & 9631.6 & 9500 & 9500 & 10000\\
\hline
\cellcolor{gray!10}{R3D Frechet} & \cellcolor{gray!10}{200} & \cellcolor{gray!10}{4368.4} & \cellcolor{gray!10}{5500} & \cellcolor{gray!10}{4000} & \cellcolor{gray!10}{3000} & \cellcolor{gray!10}{10000.0} & \cellcolor{gray!10}{10000} & \cellcolor{gray!10}{10000} & \cellcolor{gray!10}{10000}\\
\hline
R3D Frechet & 500 & 3684.2 & 4500 & 4000 & 2000 & 10000.0 & 10000 & 10000 & 10000\\
\hline
\cellcolor{gray!10}{R3D Simple} & \cellcolor{gray!10}{100} & \cellcolor{gray!10}{5578.9} & \cellcolor{gray!10}{7000} & \cellcolor{gray!10}{5500} & \cellcolor{gray!10}{5000} & \cellcolor{gray!10}{9736.8} & \cellcolor{gray!10}{9500} & \cellcolor{gray!10}{9500} & \cellcolor{gray!10}{10000}\\
\hline
R3D Simple & 200 & 5394.7 & 7000 & 5500 & 4000 & 10000.0 & 10000 & 10000 & 10000\\
\hline
\cellcolor{gray!10}{R3D Simple} & \cellcolor{gray!10}{500} & \cellcolor{gray!10}{3868.4} & \cellcolor{gray!10}{5000} & \cellcolor{gray!10}{4000} & \cellcolor{gray!10}{3500} & \cellcolor{gray!10}{10000.0} & \cellcolor{gray!10}{10000} & \cellcolor{gray!10}{10000} & \cellcolor{gray!10}{10000}\\
\hline
\end{tabular}
\end{table}

==> tabs/coverage_power_table_scenario_4.tex <==
\begin{table}[!h]
\centering
\caption{Coverage and Power for Scenario 4}
\centering
\begin{tabular}[t]{r|r|r|r|r|r|r|r|r|r}
\hline
\multicolumn{2}{c|}{ } & \multicolumn{4}{c|}{Coverage (\%)} & \multicolumn{4}{c}{Power (\%)} \\
\cline{3-6} \cline{7-10}
Method & Sample\_Size & Average & Q25 & Q50 & Q75 & Average & Q25 & Q50 & Q75\\
\hline
\cellcolor{gray!10}{Classical QTE.RD} & \cellcolor{gray!10}{100} & \cellcolor{gray!10}{NaN} & \cellcolor{gray!10}{NaN} & \cellcolor{gray!10}{NaN} & \cellcolor{gray!10}{NaN} & \cellcolor{gray!10}{NaN} & \cellcolor{gray!10}{NaN} & \cellcolor{gray!10}{NaN} & \cellcolor{gray!10}{NaN}\\
\hline
Classical QTE.RD & 200 & NaN & NaN & NaN & NaN & NaN & NaN & NaN & NaN\\
\hline
\cellcolor{gray!10}{Classical QTE.RD} & \cellcolor{gray!10}{500} & \cellcolor{gray!10}{NaN} & \cellcolor{gray!10}{NaN} & \cellcolor{gray!10}{NaN} & \cellcolor{gray!10}{NaN} & \cellcolor{gray!10}{NaN} & \cellcolor{gray!10}{NaN} & \cellcolor{gray!10}{NaN} & \cellcolor{gray!10}{NaN}\\
\hline
R3D Frechet & 100 & 5868.4 & 7000 & 8000 & 5000 & 10000 & 10000 & 10000 & 10000\\
\hline
\cellcolor{gray!10}{R3D Frechet} & \cellcolor{gray!10}{200} & \cellcolor{gray!10}{3657.9} & \cellcolor{gray!10}{4500} & \cellcolor{gray!10}{3500} & \cellcolor{gray!10}{5000} & \cellcolor{gray!10}{10000} & \cellcolor{gray!10}{10000} & \cellcolor{gray!10}{10000} & \cellcolor{gray!10}{10000}\\
\hline
R3D Frechet & 500 & 2710.5 & 2500 & 3000 & 2000 & 10000 & 10000 & 10000 & 10000\\
\hline
\cellcolor{gray!10}{R3D Simple} & \cellcolor{gray!10}{100} & \cellcolor{gray!10}{6052.6} & \cellcolor{gray!10}{6000} & \cellcolor{gray!10}{7000} & \cellcolor{gray!10}{6500} & \cellcolor{gray!10}{10000} & \cellcolor{gray!10}{10000} & \cellcolor{gray!10}{10000} & \cellcolor{gray!10}{10000}\\
\hline
R3D Simple & 200 & 4657.9 & 4000 & 4000 & 6000 & 10000 & 10000 & 10000 & 10000\\
\hline
\cellcolor{gray!10}{R3D Simple} & \cellcolor{gray!10}{500} & \cellcolor{gray!10}{3421.1} & \cellcolor{gray!10}{5000} & \cellcolor{gray!10}{3500} & \cellcolor{gray!10}{4000} & \cellcolor{gray!10}{10000} & \cellcolor{gray!10}{10000} & \cellcolor{gray!10}{10000} & \cellcolor{gray!10}{10000}\\
\hline
\end{tabular}
\end{table}

==> tabs/delta_mu_sim_20250329_193606/joint_treatment_nullity_scenario_2_frechet.tex <==
\hline
n & $\delta_{\mu} = 5$ \\
\hline
500 & 87.3333333333333 \\
\hline
\end{tabular}
\end{table}


==> tabs/delta_mu_sim_20250329_193606/joint_treatment_nullity_scenario_2_local_poly.tex <==
\hline
n & $\delta_{\mu} = 5$ \\
\hline
500 & 86.3333333333333 \\
\hline
\end{tabular}
\end{table}


==> tabs/delta_mu_sim_20250329_193606/treatment_homogeneity_scenario_2_frechet.tex <==
\hline
n & $\delta_{\mu} = 5$ \\
\hline
500 & 84 \\
\hline
\end{tabular}
\end{table}


==> tabs/delta_mu_sim_20250329_193606/treatment_homogeneity_scenario_2_local_poly.tex <==
\hline
n & $\delta_{\mu} = 5$ \\
\hline
500 & 84.3333333333333 \\
\hline
\end{tabular}
\end{table}


==> tabs/delta_mu_sim_20250329_193748/joint_treatment_nullity_scenario_2_frechet.tex <==
\hline
n & $\delta_{\mu} = 5$ \\
\hline
500 & 87.3333333333333 \\
\hline
\end{tabular}
\end{table}


==> tabs/delta_mu_sim_20250329_193748/joint_treatment_nullity_scenario_2_local_poly.tex <==
\hline
n & $\delta_{\mu} = 5$ \\
\hline
500 & 86.3333333333333 \\
\hline
\end{tabular}
\end{table}


==> tabs/delta_mu_sim_20250329_193748/treatment_homogeneity_scenario_2_frechet.tex <==
\hline
n & $\delta_{\mu} = 5$ \\
\hline
500 & 84 \\
\hline
\end{tabular}
\end{table}


==> tabs/delta_mu_sim_20250329_193748/treatment_homogeneity_scenario_2_local_poly.tex <==
\hline
n & $\delta_{\mu} = 5$ \\
\hline
500 & 84.3333333333333 \\
\hline
\end{tabular}
\end{table}


==> tabs/delta_mu_sim_20250329_194128/joint_treatment_nullity_scenario_1_frechet.tex <==
\hline
n & $\delta_{\mu} = 5$ \\
\hline
1000 & 91.3333333333333 \\
\hline
\end{tabular}
\end{table}


==> tabs/delta_mu_sim_20250329_194128/joint_treatment_nullity_scenario_1_local_poly.tex <==
\hline
n & $\delta_{\mu} = 5$ \\
\hline
1000 & 92 \\
\hline
\end{tabular}
\end{table}


==> tabs/delta_mu_sim_20250329_194128/treatment_homogeneity_scenario_1_frechet.tex <==
\hline
n & $\delta_{\mu} = 5$ \\
\hline
1000 & 88.6666666666667 \\
\hline
\end{tabular}
\end{table}


==> tabs/delta_mu_sim_20250329_194128/treatment_homogeneity_scenario_1_local_poly.tex <==
\hline
n & $\delta_{\mu} = 5$ \\
\hline
1000 & 89.3333333333333 \\
\hline
\end{tabular}
\end{table}


==> tabs/delta_mu_sim_20250329_194617/joint_treatment_nullity_scenario_1_frechet.tex <==
\hline
n & $\delta_{\mu} = 5$ \\
\hline
1000 & 89.8 \\
\hline
\end{tabular}
\end{table}


==> tabs/delta_mu_sim_20250329_194617/joint_treatment_nullity_scenario_1_local_poly.tex <==
\hline
n & $\delta_{\mu} = 5$ \\
\hline
1000 & 89.9 \\
\hline
\end{tabular}
\end{table}


==> tabs/delta_mu_sim_20250329_194617/treatment_homogeneity_scenario_1_frechet.tex <==
\hline
n & $\delta_{\mu} = 5$ \\
\hline
1000 & 90.1 \\
\hline
\end{tabular}
\end{table}


==> tabs/delta_mu_sim_20250329_194617/treatment_homogeneity_scenario_1_local_poly.tex <==
\hline
n & $\delta_{\mu} = 5$ \\
\hline
1000 & 90.6 \\
\hline
\end{tabular}
\end{table}


==> tabs/package_cites.tex <==
\item \bibentry{NULL}
\item \bibentry{NULL}
\item \bibentry{NULL}
\item \bibentry{NULL}
\item \bibentry{NULL}
\item \bibentry{NULL}
\item \bibentry{NULL}
\item \bibentry{NULL}
\item \bibentry{NULL}
\item \bibentry{NULL}
\item \bibentry{NULL}
\item \bibentry{NULL}
\item \bibentry{NULL}
\item \bibentry{NULL}
\item \bibentry{NULL}
\item \bibentry{NULL}
\item \bibentry{NULL}
\item \bibentry{NULL}
\item \bibentry{NULL}
\item \bibentry{NULL}
\item \bibentry{NULL}
\item \bibentry{NULL}

==> tabs/simulation_coverage_table.tex <==
% latex table generated in R 4.4.0 by xtable 1.8-4 package
% Thu Mar 27 20:59:32 2025
\begin{table}[htbp!]
\centering
\caption{Simulation Results Across Scenarios} 
\label{tab:simulation_results}
\scriptsize
\begin{tabular}{ccccc}
  \hline
Method & Sample\_Size & Uniform Confidence Band Coverage (\%) & Acceptance Probability (Homogeneity Test) (\%) & Scenario \\ 
  \hline
R3D Frechet & 200.00 & 85.10 & 87.30 & Scenario 1 \\ 
  R3D Frechet & 500.00 & 90.40 & 90.60 & Scenario 1 \\ 
  R3D Frechet & 1000.00 & 91.90 & 93.80 & Scenario 1 \\ 
  R3D Frechet & 2000.00 & 93.80 & 94.90 & Scenario 1 \\ 
  R3D Frechet & 5000.00 & 93.50 & 95.20 & Scenario 1 \\ 
  R3D Local Polynomial & 200.00 & 84.40 & 82.80 & Scenario 1 \\ 
  R3D Local Polynomial & 500.00 & 90.60 & 86.00 & Scenario 1 \\ 
  R3D Local Polynomial & 1000.00 & 91.50 & 89.20 & Scenario 1 \\ 
  R3D Local Polynomial & 2000.00 & 93.60 & 88.30 & Scenario 1 \\ 
  R3D Local Polynomial & 5000.00 & 93.30 & 92.00 & Scenario 1 \\ 
  R3D Frechet & 200.00 & 88.40 & 47.20 & Scenario 2 \\ 
  R3D Frechet & 500.00 & 92.20 & 13.60 & Scenario 2 \\ 
  R3D Frechet & 1000.00 & 92.80 & 1.20 & Scenario 2 \\ 
  R3D Frechet & 2000.00 & 93.70 & 0.00 & Scenario 2 \\ 
  R3D Frechet & 5000.00 & 92.30 & 0.00 & Scenario 2 \\ 
  R3D Local Polynomial & 200.00 & 86.60 & 61.00 & Scenario 2 \\ 
  R3D Local Polynomial & 500.00 & 91.40 & 32.30 & Scenario 2 \\ 
  R3D Local Polynomial & 1000.00 & 93.30 & 12.80 & Scenario 2 \\ 
  R3D Local Polynomial & 2000.00 & 93.00 & 3.60 & Scenario 2 \\ 
  R3D Local Polynomial & 5000.00 & 92.40 & 0.60 & Scenario 2 \\ 
   \hline
\end{tabular}
\end{table}


==> tabs/simulation_scenario_1.tex <==
% latex table generated in R 4.4.0 by xtable 1.8-4 package
% Thu Mar 27 22:01:18 2025
\begin{table}[htbp!]
\centering
\caption{Normal Distributions} 
\label{tab:simulation_results_scenario_1}
\begin{tabular}{cccc}
  \hline
Method & Sample\_Size & Uniform Band & Homogeneity \\ 
  \hline
R3D Frechet & 100.00 & 70.00 & 80.00 \\ 
  R3D Frechet & 200.00 & 70.00 & 90.00 \\ 
  R3D Local Polynomial & 100.00 & 60.00 & 90.00 \\ 
  R3D Local Polynomial & 200.00 & 80.00 & 85.00 \\ 
   \hline
\end{tabular}
\end{table}


==> tabs/simulation_scenario_2.tex <==
% latex table generated in R 4.4.0 by xtable 1.8-4 package
% Thu Mar 27 22:01:18 2025
\begin{table}[htbp!]
\centering
\caption{Normal-Exponential Distributions} 
\label{tab:simulation_results_scenario_2}
\begin{tabular}{cccc}
  \hline
Method & Sample\_Size & Uniform Band & Homogeneity \\ 
  \hline
R3D Frechet & 100.00 & 80.00 & 70.00 \\ 
  R3D Frechet & 200.00 & 85.00 & 60.00 \\ 
  R3D Local Polynomial & 100.00 & 80.00 & 70.00 \\ 
  R3D Local Polynomial & 200.00 & 95.00 & 70.00 \\ 
   \hline
\end{tabular}
\end{table}


==> tabs/stacked_cp_table.tex <==
\begin{table}[!h]
\centering
\caption{Combined Coverage and Power Metrics for All Scenarios}
\centering
\begin{tabular}[t]{l|r|r|r|r}
\hline
Scenario & Sample Size & Joint Coverage (\%) & Power Nullity (\%) & Power Homogeneity (\%)\\
\hline
\cellcolor{gray!10}{Scenario 1} & \cellcolor{gray!10}{100} & \cellcolor{gray!10}{77.4} & \cellcolor{gray!10}{66.2} & \cellcolor{gray!10}{21.0}\\
\hline
Scenario 1 & 200 & 87.0 & 79.8 & 12.2\\
\hline
\end{tabular}
\end{table}

==> tabs/standard_rd_results__David_Van_Dijcke_s_conflicted_copy_2025-04-02_.tex <==

\begin{tabular}{lcc}
\hline\hline
\multicolumn{1}{c}{Level:} & \multicolumn{1}{c}{State} & \multicolumn{1}{c}{Family} \\
\hline
Treatment Effect & -0.609 & -0.525 \\
 & (0.425) & (0.062) \\
\\
\hline 
Robust 95\% CI & [-1.542, 0.125] & [-0.681, -0.438] \\
p-value & 0.096 & 0 \\
Bandwidth & 0.088 & 0.036 \\
Effective Observations & 216 & 138692 \\
\hline\hline
\end{tabular}

==> tabs/summary_table_scenario_1.tex <==
\begin{table}[!h]
\centering
\caption{Performance Metrics for Scenario 1}
\centering
\begin{tabular}[t]{l|r|r|r|r|r|r}
\hline
\multicolumn{2}{c|}{ } & \multicolumn{5}{c}{Performance Metrics} \\
\cline{3-7}
Method & Sample Size & Abs. Bias & Rel. Bias & MSE & RMSE & SE\\
\hline
\cellcolor{gray!10}{Quantile RD} & \cellcolor{gray!10}{200} & \cellcolor{gray!10}{NaN} & \cellcolor{gray!10}{NaN} & \cellcolor{gray!10}{NaN} & \cellcolor{gray!10}{NaN} & \cellcolor{gray!10}{NaN}\\
\hline
Quantile RD & 500 & NaN & NaN & NaN & NaN & NaN\\
\hline
\cellcolor{gray!10}{R3D Frechet} & \cellcolor{gray!10}{200} & \cellcolor{gray!10}{0.6260} & \cellcolor{gray!10}{0.6260} & \cellcolor{gray!10}{0.6333} & \cellcolor{gray!10}{0.7958} & \cellcolor{gray!10}{0.7964}\\
\hline
R3D Frechet & 500 & 0.3859 & 0.3859 & 0.2447 & 0.4947 & 0.4950\\
\hline
\cellcolor{gray!10}{R3D Local Polynomial} & \cellcolor{gray!10}{200} & \cellcolor{gray!10}{0.6217} & \cellcolor{gray!10}{0.6217} & \cellcolor{gray!10}{0.6351} & \cellcolor{gray!10}{0.7969} & \cellcolor{gray!10}{0.7973}\\
\hline
R3D Local Polynomial & 500 & 0.3844 & 0.3844 & 0.2435 & 0.4934 & 0.4937\\
\hline
\end{tabular}
\end{table}

==> tabs/summary_table_scenario_2.tex <==
\begin{table}[!h]
\centering
\caption{Performance Metrics for Scenario 2}
\centering
\begin{tabular}[t]{l|r|r|r|r|r|r}
\hline
\multicolumn{2}{c|}{ } & \multicolumn{5}{c}{Performance Metrics} \\
\cline{3-7}
Method & Sample Size & Abs. Bias & Rel. Bias & MSE & RMSE & SE\\
\hline
\cellcolor{gray!10}{Quantile RD} & \cellcolor{gray!10}{200} & \cellcolor{gray!10}{NaN} & \cellcolor{gray!10}{NaN} & \cellcolor{gray!10}{NaN} & \cellcolor{gray!10}{NaN} & \cellcolor{gray!10}{NaN}\\
\hline
Quantile RD & 500 & NaN & NaN & NaN & NaN & NaN\\
\hline
\cellcolor{gray!10}{R3D Frechet} & \cellcolor{gray!10}{200} & \cellcolor{gray!10}{1.0582} & \cellcolor{gray!10}{0.2819} & \cellcolor{gray!10}{1.8819} & \cellcolor{gray!10}{1.3718} & \cellcolor{gray!10}{1.2096}\\
\hline
R3D Frechet & 500 & 0.7610 & 0.1991 & 1.0305 & 1.0151 & 0.7839\\
\hline
\cellcolor{gray!10}{R3D Local Polynomial} & \cellcolor{gray!10}{200} & \cellcolor{gray!10}{1.0612} & \cellcolor{gray!10}{0.2826} & \cellcolor{gray!10}{1.8884} & \cellcolor{gray!10}{1.3742} & \cellcolor{gray!10}{1.2134}\\
\hline
R3D Local Polynomial & 500 & 0.7637 & 0.2002 & 1.0372 & 1.0185 & 0.7883\\
\hline
\end{tabular}
\end{table}

==> tabs/summary_table_scenario_3.tex <==
\begin{table}[!h]
\centering
\caption{Performance Metrics for Scenario 3}
\centering
\begin{tabular}[t]{l|r|r|r|r|r|r}
\hline
\multicolumn{2}{c|}{ } & \multicolumn{5}{c}{Performance Metrics} \\
\cline{3-7}
Method & Sample Size & Abs. Bias & Rel. Bias & MSE & RMSE & SE\\
\hline
\cellcolor{gray!10}{Classical QTE.RD} & \cellcolor{gray!10}{100} & \cellcolor{gray!10}{NaN} & \cellcolor{gray!10}{NaN} & \cellcolor{gray!10}{NaN} & \cellcolor{gray!10}{NaN} & \cellcolor{gray!10}{NaN}\\
\hline
Classical QTE.RD & 200 & NaN & NaN & NaN & NaN & NaN\\
\hline
\cellcolor{gray!10}{Classical QTE.RD} & \cellcolor{gray!10}{500} & \cellcolor{gray!10}{NaN} & \cellcolor{gray!10}{NaN} & \cellcolor{gray!10}{NaN} & \cellcolor{gray!10}{NaN} & \cellcolor{gray!10}{NaN}\\
\hline
R3D Frechet & 100 & 2.0986 & 0.1899 & 8.8238 & 2.9705 & 2.8992\\
\hline
\cellcolor{gray!10}{R3D Frechet} & \cellcolor{gray!10}{200} & \cellcolor{gray!10}{1.6651} & \cellcolor{gray!10}{0.1525} & \cellcolor{gray!10}{4.8446} & \cellcolor{gray!10}{2.2010} & \cellcolor{gray!10}{2.0621}\\
\hline
R3D Frechet & 500 & 0.9074 & 0.0770 & 1.6047 & 1.2668 & 1.0802\\
\hline
\cellcolor{gray!10}{R3D Simple} & \cellcolor{gray!10}{100} & \cellcolor{gray!10}{2.0774} & \cellcolor{gray!10}{0.1827} & \cellcolor{gray!10}{8.0685} & \cellcolor{gray!10}{2.8405} & \cellcolor{gray!10}{2.6843}\\
\hline
R3D Simple & 200 & 1.5420 & 0.1403 & 4.3061 & 2.0751 & 1.9707\\
\hline
\cellcolor{gray!10}{R3D Simple} & \cellcolor{gray!10}{500} & \cellcolor{gray!10}{0.8954} & \cellcolor{gray!10}{0.0752} & \cellcolor{gray!10}{1.6538} & \cellcolor{gray!10}{1.2860} & \cellcolor{gray!10}{1.0828}\\
\hline
\end{tabular}
\end{table}

==> tabs/summary_table_scenario_4.tex <==
\begin{table}[!h]
\centering
\caption{Performance Metrics for Scenario 4}
\centering
\begin{tabular}[t]{l|r|r|r|r|r|r}
\hline
\multicolumn{2}{c|}{ } & \multicolumn{5}{c}{Performance Metrics} \\
\cline{3-7}
Method & Sample Size & Abs. Bias & Rel. Bias & MSE & RMSE & SE\\
\hline
\cellcolor{gray!10}{Classical QTE.RD} & \cellcolor{gray!10}{100} & \cellcolor{gray!10}{NaN} & \cellcolor{gray!10}{NaN} & \cellcolor{gray!10}{NaN} & \cellcolor{gray!10}{NaN} & \cellcolor{gray!10}{NaN}\\
\hline
Classical QTE.RD & 200 & NaN & NaN & NaN & NaN & NaN\\
\hline
\cellcolor{gray!10}{Classical QTE.RD} & \cellcolor{gray!10}{500} & \cellcolor{gray!10}{NaN} & \cellcolor{gray!10}{NaN} & \cellcolor{gray!10}{NaN} & \cellcolor{gray!10}{NaN} & \cellcolor{gray!10}{NaN}\\
\hline
R3D Frechet & 100 & 0.0724 & 0.0241 & 0.0107 & 0.1035 & 0.1027\\
\hline
\cellcolor{gray!10}{R3D Frechet} & \cellcolor{gray!10}{200} & \cellcolor{gray!10}{0.0333} & \cellcolor{gray!10}{0.0111} & \cellcolor{gray!10}{0.0018} & \cellcolor{gray!10}{0.0429} & \cellcolor{gray!10}{0.0421}\\
\hline
R3D Frechet & 500 & 0.0117 & 0.0039 & 0.0002 & 0.0147 & 0.0145\\
\hline
\cellcolor{gray!10}{R3D Simple} & \cellcolor{gray!10}{100} & \cellcolor{gray!10}{0.0632} & \cellcolor{gray!10}{0.0211} & \cellcolor{gray!10}{0.0090} & \cellcolor{gray!10}{0.0946} & \cellcolor{gray!10}{0.0913}\\
\hline
R3D Simple & 200 & 0.0291 & 0.0097 & 0.0016 & 0.0401 & 0.0393\\
\hline
\cellcolor{gray!10}{R3D Simple} & \cellcolor{gray!10}{500} & \cellcolor{gray!10}{0.0109} & \cellcolor{gray!10}{0.0036} & \cellcolor{gray!10}{0.0002} & \cellcolor{gray!10}{0.0141} & \cellcolor{gray!10}{0.0140}\\
\hline
\end{tabular}
\end{table}
